Online Gradient Descent for Linear Dynamical Systems

In this paper, online convex optimization is applied to the problem of controlling linear dynamical systems. An algorithm similar to online gradient descent, which can handle time-varying and unknown cost functions, is proposed. Then, performance guarantees are derived in terms of regret analysis. We show that the proposed control scheme achieves sublinear regret if the variation of the cost functions is sublinear. In addition, as a special case, the system converges to the optimal equilibrium if the cost functions are invariant after some finite time. Finally, the performance of the resulting closed loop is illustrated by numerical simulations.

==> figures/StatesInputs_old.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\fwidth,
height=0.113\hwidth,
at={(0\fwidth,0.469\hwidth)},
scale only axis,
xmin=0,
xmax=30,
ymin=-4,
ymax=4,
ylabel style={font=\color{white!15!black}},
ylabel={$\text{x}_\text{1}$},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
0	-1.1162\\
1	-3.116295\\
2	0.457610910122201\\
3	-2.48398538148877\\
4	-1.14117720072036\\
5	-1.11646313539575\\
6	-1.11618617876424\\
7	-1.11618515868864\\
8	-1.1161852133997\\
9	2.74357019612011\\
10	-0.314735806363381\\
11	2.34243434377085\\
12	2.37543644102043\\
13	1.66982429616596\\
14	2.22968596280111\\
15	1.74328065689241\\
16	1.73723957524613\\
17	1.73706899237735\\
18	1.73706420941288\\
19	1.73706409057781\\
20	1.73706408782262\\
21	-2.59271513986938\\
22	0.838018390192139\\
23	-2.14273061029474\\
24	-2.17975111293223\\
25	-2.18079646549849\\
26	-2.1808257760733\\
27	-2.18082650430862\\
28	-2.18082652119278\\
29	-2.18082652156828\\
30	-2.18082652157641\\
31	-2.18082652157657\\
32	-2.18082652157659\\
33	-2.18082652157658\\
34	-2.18082652157658\\
35	-2.18082652157659\\
36	-2.18082652157657\\
37	-2.18082652157659\\
38	-2.18082652157658\\
39	-2.18082652157658\\
40	-2.18082652157658\\
41	-2.18082652157658\\
42	-2.18082652157658\\
43	-2.18082652157658\\
44	-2.18082652157659\\
45	-2.18082652157658\\
46	2.79668004042331\\
47	-4.27600788655203\\
48	1.6297231640904\\
49	-0.481624048756047\\
50	-0.50717353577864\\
};


\addplot [color=mycolor2, dashed]
  table[row sep=crcr]{%
1	-1.1162\\
2	-1.1162\\
3	-1.1162\\
4	-1.1162\\
5	-1.1162\\
6	-1.1162\\
7	-1.1162\\
8	2.37639511612951\\
9	2.37639511612951\\
10	2.37639511612951\\
11	2.37639511612951\\
12	1.73706408775998\\
13	1.73706408775998\\
14	1.73706408775998\\
15	1.73706408775998\\
16	1.73706408775998\\
17	1.73706408775998\\
18	1.73706408775998\\
19	1.73706408775998\\
20	-2.18082652157658\\
21	-2.18082652157658\\
22	-2.18082652157658\\
23	-2.18082652157658\\
24	-2.18082652157658\\
25	-2.18082652157658\\
26	-2.18082652157658\\
27	-2.18082652157658\\
28	-2.18082652157658\\
29	-2.18082652157658\\
30	-2.18082652157658\\
31	-2.18082652157658\\
32	-2.18082652157658\\
33	-2.18082652157658\\
34	-2.18082652157658\\
35	-2.18082652157658\\
36	-2.18082652157658\\
37	-2.18082652157658\\
38	-2.18082652157658\\
39	-2.18082652157658\\
40	-2.18082652157658\\
41	-2.18082652157658\\
42	-2.18082652157658\\
43	-2.18082652157658\\
44	-2.18082652157658\\
45	2.32317361143755\\
46	-0.507916079672065\\
47	-0.507916079672065\\
48	-0.507916079672065\\
49	-0.507916079672065\\
50	-0.507916079672065\\
};


\end{axis}

\begin{axis}[%
width=0.951\fwidth,
height=0.113\hwidth,
at={(0\fwidth,0.313\hwidth)},
scale only axis,
xmin=0,
xmax=30,
ymin=-5,
ymax=5,
ylabel style={font=\color{white!15!black}},
ylabel={$\text{x}_\text{2}$},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
0	-2.1628\\
1	-2.162825\\
2	-4.962895175\\
3	-2.87499735670392\\
4	-2.17525604176426\\
5	-2.16284045523763\\
6	-2.1627067839967\\
7	-2.16270644554975\\
8	-2.16270647753221\\
9	-2.16270647880417\\
10	3.24095109773571\\
11	4.58588114596025\\
12	4.60394943182854\\
13	4.60445895908604\\
14	3.61531138878983\\
15	3.36911693367244\\
16	3.36580950622966\\
17	3.36571623618984\\
18	3.36571366124891\\
19	3.36571359779265\\
20	3.36571359632828\\
21	3.36571359629581\\
22	-2.69597732238789\\
23	-4.20468604937861\\
24	-4.22495437624903\\
25	-4.22552594636195\\
26	-4.22554172590572\\
27	-4.22554211477311\\
28	-4.22554212374699\\
29	-4.22554212394597\\
30	-4.22554212395027\\
31	-4.22554212395037\\
32	-4.22554212395036\\
33	-4.22554212395037\\
34	-4.22554212395038\\
35	-4.22554212395038\\
36	-4.22554212395038\\
37	-4.22554212395037\\
38	-4.22554212395037\\
39	-4.22554212395037\\
40	-4.22554212395037\\
41	-4.22554212395037\\
42	-4.22554212395037\\
43	-4.22554212395037\\
44	-4.22554212395037\\
45	-4.22554212395037\\
46	-4.22554212395038\\
47	2.74296706284947\\
48	0.0971641558393412\\
49	-0.969736784934501\\
50	-0.983725715422661\\
};


\addplot [color=mycolor2, dashed]
  table[row sep=crcr]{%
1	-2.1628\\
2	-2.1628\\
3	-2.1628\\
4	-2.1628\\
5	-2.1628\\
6	-2.1628\\
7	-2.1628\\
8	4.60447338062262\\
9	4.60447338062262\\
10	4.60447338062262\\
11	4.60447338062262\\
12	3.36571359629509\\
13	3.36571359629509\\
14	3.36571359629509\\
15	3.36571359629509\\
16	3.36571359629509\\
17	3.36571359629509\\
18	3.36571359629509\\
19	3.36571359629509\\
20	-4.22554212395036\\
21	-4.22554212395036\\
22	-4.22554212395036\\
23	-4.22554212395036\\
24	-4.22554212395036\\
25	-4.22554212395036\\
26	-4.22554212395036\\
27	-4.22554212395036\\
28	-4.22554212395036\\
29	-4.22554212395036\\
30	-4.22554212395036\\
31	-4.22554212395036\\
32	-4.22554212395036\\
33	-4.22554212395036\\
34	-4.22554212395036\\
35	-4.22554212395036\\
36	-4.22554212395036\\
37	-4.22554212395036\\
38	-4.22554212395036\\
39	-4.22554212395036\\
40	-4.22554212395036\\
41	-4.22554212395036\\
42	-4.22554212395036\\
43	-4.22554212395036\\
44	-4.22554212395036\\
45	4.5013520604484\\
46	-0.984131827475428\\
47	-0.984131827475428\\
48	-0.984131827475428\\
49	-0.984131827475428\\
50	-0.984131827475428\\
};


\end{axis}

\begin{axis}[%
width=0.951\fwidth,
height=0.113\hwidth,
at={(0\fwidth,0.156\hwidth)},
scale only axis,
xmin=0,
xmax=30,
ymin=-4,
ymax=4,
ylabel style={font=\color{white!15!black}},
ylabel={$\text{x}_\text{3}$},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
0	-0.2459\\
1	-2.2459185\\
2	0.417967092622199\\
3	0.672987610904334\\
4	-0.229284957857637\\
5	-0.245672731373191\\
6	-0.245853842080547\\
7	-0.245854438196538\\
8	-0.245854399849263\\
9	3.61390101357771\\
10	2.3117837235928\\
11	0.546648199368159\\
12	0.524087240427535\\
13	-0.183093701169982\\
14	0.0552465471801575\\
15	0.37836135499677\\
16	0.382491171898034\\
17	0.382607760556137\\
18	0.38261101107039\\
19	0.382611091591607\\
20	0.382611093455339\\
21	-3.94716813413398\\
22	-2.48648415264222\\
23	-0.506398502934131\\
24	-0.481090469963197\\
25	-0.48037600050274\\
26	-0.480356080965195\\
27	-0.480355587521714\\
28	-0.480355576100576\\
29	-0.480355575846851\\
30	-0.480355575841368\\
31	-0.480355575841241\\
32	-0.480355575841247\\
33	-0.480355575841255\\
34	-0.480355575841247\\
35	-0.48035557584125\\
36	-0.480355575841236\\
37	-0.480355575841243\\
38	-0.480355575841245\\
39	-0.480355575841247\\
40	-0.48035557584125\\
41	-0.480355575841245\\
42	-0.480355575841243\\
43	-0.480355575841244\\
44	-0.48035557584125\\
45	-0.480355575841249\\
46	4.49715098615864\\
47	-0.310771455106741\\
48	-1.53157600138446\\
49	-0.129849094194185\\
50	-0.112382720697618\\
};


\addplot [color=mycolor2, dashed]
  table[row sep=crcr]{%
1	-0.2459\\
2	-0.2459\\
3	-0.2459\\
4	-0.2459\\
5	-0.2459\\
6	-0.2459\\
7	-0.2459\\
8	0.52343211765853\\
9	0.52343211765853\\
10	0.52343211765853\\
11	0.52343211765853\\
12	0.38261109349765\\
13	0.38261109349765\\
14	0.38261109349765\\
15	0.38261109349765\\
16	0.38261109349765\\
17	0.38261109349765\\
18	0.38261109349765\\
19	0.38261109349765\\
20	-0.480355575841245\\
21	-0.480355575841245\\
22	-0.480355575841245\\
23	-0.480355575841245\\
24	-0.480355575841245\\
25	-0.480355575841245\\
26	-0.480355575841245\\
27	-0.480355575841245\\
28	-0.480355575841245\\
29	-0.480355575841245\\
30	-0.480355575841245\\
31	-0.480355575841245\\
32	-0.480355575841245\\
33	-0.480355575841245\\
34	-0.480355575841245\\
35	-0.480355575841245\\
36	-0.480355575841245\\
37	-0.480355575841245\\
38	-0.480355575841245\\
39	-0.480355575841245\\
40	-0.480355575841245\\
41	-0.480355575841245\\
42	-0.480355575841245\\
43	-0.480355575841245\\
44	-0.480355575841245\\
45	0.511709384887028\\
46	-0.111875162245148\\
47	-0.111875162245148\\
48	-0.111875162245148\\
49	-0.111875162245148\\
50	-0.111875162245148\\
};


\end{axis}

\begin{axis}[%
width=0.951\fwidth,
height=0.113\hwidth,
at={(0\fwidth,0\hwidth)},
scale only axis,
xmin=0,
xmax=30,
ymin=-10,
ymax=10,
ylabel style={font=\color{white!15!black}},
ylabel={$\text{u}_\text{t}$},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	0\\
2	9.1740555351222\\
3	-0.221892626705925\\
4	2.30177728045301\\
5	2.00570083084647\\
6	2.00001571197072\\
7	1.99994930145246\\
8	1.99994898195213\\
9	5.85970440419856\\
10	-8.00591675088757\\
11	-3.64138034425\\
12	-4.25087077100541\\
13	-4.96430123993366\\
14	-2.4263368424859\\
15	-3.22528903376692\\
16	-3.11371933930596\\
17	-3.11245876681341\\
18	-3.11242317888946\\
19	-3.11242216155313\\
20	-3.11242213602425\\
21	-7.44220136305977\\
22	8.11191400438239\\
23	3.21588147279893\\
24	3.89959364257701\\
25	3.90731858889026\\
26	3.90753667603328\\
27	3.90754291039144\\
28	3.90754306683544\\
29	3.90754307048305\\
30	3.90754307056446\\
31	3.90754307056624\\
32	3.90754307056624\\
33	3.90754307056627\\
34	3.90754307056628\\
35	3.90754307056627\\
36	3.9075430705663\\
37	3.90754307056624\\
38	3.90754307056627\\
39	3.90754307056626\\
40	3.90754307056627\\
41	3.90754307056628\\
42	3.90754307056627\\
43	3.90754307056626\\
44	3.90754307056626\\
45	3.90754307056628\\
46	8.88504963256616\\
47	-12.1246566680089\\
48	4.74330454741219\\
49	0.419409722284295\\
50	0.904583379709183\\
};


\addplot [color=mycolor2, dashed]
  table[row sep=crcr]{%
1	2\\
2	2\\
3	2\\
4	2\\
5	2\\
6	2\\
7	2\\
8	-4.25795732814473\\
9	-4.25795732814473\\
10	-4.25795732814473\\
11	-4.25795732814473\\
12	-3.11242213541545\\
13	-3.11242213541545\\
14	-3.11242213541545\\
15	-3.11242213541545\\
16	-3.11242213541545\\
17	-3.11242213541545\\
18	-3.11242213541545\\
19	-3.11242213541545\\
20	3.90754307056626\\
21	3.90754307056626\\
22	3.90754307056626\\
23	3.90754307056626\\
24	3.90754307056626\\
25	3.90754307056626\\
26	3.90754307056626\\
27	3.90754307056626\\
28	3.90754307056626\\
29	3.90754307056626\\
30	3.90754307056626\\
31	3.90754307056626\\
32	3.90754307056626\\
33	3.90754307056626\\
34	3.90754307056626\\
35	3.90754307056626\\
36	3.90754307056626\\
37	3.90754307056626\\
38	3.90754307056626\\
39	3.90754307056626\\
40	3.90754307056626\\
41	3.90754307056626\\
42	3.90754307056626\\
43	3.90754307056626\\
44	3.90754307056626\\
45	-4.16259654643805\\
46	0.910069617145413\\
47	0.910069617145413\\
48	0.910069617145413\\
49	0.910069617145413\\
50	0.910069617145413\\
};


\end{axis}

\begin{axis}[%
width=1.227\fwidth,
height=0.714\hwidth,
at={(-0.16\fwidth,-0.079\hwidth)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%
